Push--Pull with Device Sampling

We consider decentralized optimization problems in which a number of agents collaborate to minimize the average of their local functions by exchanging over an underlying communication graph. Specifically, we place ourselves in an asynchronous model where only a random portion of nodes perform computation at each iteration, while the information exchange can be conducted between all the nodes and in an asymmetric fashion. For this setting, we propose an algorithm that combines gradient tracking with a network-level variance reduction (in contrast to variance reduction within each node). This enables each node to track the average of the gradients of the objective functions. Our theoretical analysis shows that the algorithm converges linearly, when the local objective functions are strongly convex, under mild connectivity conditions on the expected mixing matrices. In particular, our result does not require the mixing matrices to be doubly stochastic. In the experiments, we investigate a broadcast mechanism that transmits information from computing nodes to their neighbors, and confirm the linear convergence of our method on both synthetic and real-world datasets.

==> Response/comm_comp_trade-off.tex <==
\begin{figure}[t]
    \centering
    \begin{subfigure}[t]{0.4\textwidth}
    \includegraphics[width=\textwidth]{Content/figs/comm_comp_tradeoff_broadcast_neighbors.pdf}
    \caption{\textit{Broadcast:} We fix $\nWorkersActive=10$ and vary the number of neighbors that each active node transmits information to.}
    \label{subfig:comm-comp-trade-off-broadcast}
    \end{subfigure}
    \hspace{2em}
    \begin{subfigure}[t]{0.4\textwidth}
    \includegraphics[width=\textwidth]{Content/figs/comm_comp_tradeoff_matropolis_neighbors.pdf}
    \caption{\textit{Symmetric communication between active nodes and their neighbors:} We fix $\nWorkersActive=10$ and vary the number of neighbors that we select for each active node to add in the communication subgraph.
    }
    \label{subfig:comm-comp-trade-off-active-metrapolis}
    \end{subfigure}\\[0.4em]
    \centering
    \begin{subfigure}{0.9\textwidth}
    \centering
    \includegraphics[width=0.46\textwidth]{Content/figs/comm_comp_tradeoff_random_gossip_lr1e-3.pdf}
    \hspace{2em}
    \includegraphics[width=0.46\textwidth]{Content/figs/comm_comp_tradeoff_random_gossip_lr1e-4.pdf}
    \caption{\textit{Symmetric communication between randomly selected nodes:}
    We vary the number of active nodes $\nWorkersActive$ while independently sampling a number of nodes (at most $10$) for communication in each round.
    In the left and the right plots we fix the stepsize to be respectively $\step=10^{-3}$ and  $\step=10^{-4}$.
    }
    \label{subfig:comm-comp-trade-off-random-gossip}
    \end{subfigure}
    % \hspace{2em}
    % \begin{subfigure}{0.4\textwidth}
    % \includegraphics[width=\textwidth]{Content/figs/comm_comp_tradeoff_random_gossip_lr1e-4.pdf}
    % \caption{\textit{Symmetric communication between randomly selected nodes ($\step=10^{-4}$):}
    % We vary the number of active nodes $\nWorkersActive$ while independently sampling a number of nodes (at most $10$) for communication in each round.
    % Stepsize is fixed at $10^{-4}$
    % }
    % \end{subfigure}\\[0.4em]
    \caption{Illustration of the influence of various network parameters on the behavior of \acs{PPDS} for the ridge regression experiment.
    We plot the number of local communications and computations that are needed for the algorithm to achieve suboptimality values $10^{-2}$, $10^{-3}$, and $10^{-4}$ (from bottom left to top right). 
    Each line corresponds a specific configuration.}
    \label{fig:comm-comp-trade-off}
\end{figure}

==> Response/lambda_value.tex <==
\begin{table}[h]
    \setlength{\tabcolsep}{11pt}
    \normalsize
    \centering
    \hspace{1em}
    \begin{tabular}{c|ccccccccc}
    \toprule
        N. of selected neighbors $j$ & 2 & 4 & 6 & 8 & 10
        & 12 & 14 & 16 & 18
        \\
        Contraction factor $\cfactor$ & 0.97 & 0.94 & 0.92 & 0.91 & 0.90
        & 0.89 & 0.88 & 0.87 & 0.87
        \\
    \bottomrule
    \end{tabular}
    \vspace{0.3em}
    % \caption{Values of $\cfactor$ for different number of selected neighbors in the setup \textit{Symmetric communication between active nodes and their neighbors} that we consider in our experiment.
    % These values are obtained via Monte-Carlo estimation and rounded to the second decimal place.
    % }
    %\label{tab:lambdas}
\end{table}

